Towards Scalable and Reliable Capsule Networks for Challenging NLP Applications

Obstacles hindering the development of capsule networks for challenging NLP applications include poor scalability to large output spaces and less reliable routing processes. In this paper, we introduce: 1) an agreement score to evaluate the performance of routing processes at instance level; 2) an adaptive optimizer to enhance the reliability of routing; 3) capsule compression and partial routing to improve the scalability of capsule networks. We validate our approach on two NLP tasks, namely: multi-label text classification and question answering. Experimental results show that our approach considerably improves over strong competitors on both tasks. In addition, we gain the best results in low-resource settings with few training instances.

==> Towards Scalable and Reliable Capsule Network for Challenging NLP Applications/ack.tex <==
We thank the anonymous reviewers for helpful comments.
This work has been supported by the German Research Foundation as part of the Research Training
Group “Adaptive Preparation of Information from Heterogeneous Sources” (AIPHES) at the Technische
Universit\"at Darmstadt under grant No. GRK 1994/1.

==> ack.tex <==
We thank the anonymous reviewers for helpful comments.
This work has been supported by the German Research Foundation as part of the Research Training
Group “Adaptive Preparation of Information from Heterogeneous Sources” (AIPHES) at the Technische
Universit\"at Darmstadt under grant No. GRK 1994/1.
